Partition Functions from Rao-Blackwellized Tempered Sampling

Partition functions of probability distributions are important quantities for model evaluation and comparisons. We present a new method to compute partition functions of complex and multimodal distributions. Such distributions are often sampled using simulated tempering, which augments the target space with an auxiliary inverse temperature variable. Our method exploits the multinomial probability law of the inverse temperatures, and provides estimates of the partition function in terms of a simple quotient of Rao-Blackwellized marginal inverse temperature probability estimates, which are updated while sampling. We show that the method has interesting connections with several alternative popular methods, and offers some significant advantages. In particular, we empirically find that the new method provides more accurate estimates than Annealed Importance Sampling when calculating partition functions of large Restricted Boltzmann Machines (RBM); moreover, the method is sufficiently accurate to track training and validation log-likelihoods during learning of RBMs, at minimal computational cost.

==> sub/ais.tex <==
\section{Related Work}
\label{sec3}
In this section, we briefly review some popular estimators and explore their relation to the proposed RTS estimator (\ref{solZ}).
\subsection{AIS/RAISE}
\label{sec:ais}
Annealed Importance Sampling (AIS)~\cite{ais} is perhaps the most popular method in the machine learning literature to estimate $\log Z_K$. Here, one samples up a deterministic $\beta$ ladder, starting with a draw $x_1$ from the prior $q(x)$, then sampling the next point, $x_2$, using a transition function that leaves $f_2(x)$ invariant. The process is repeated until one has sampled $x_K$ using a transition function that leaves the (unnormalized) target distribution invariant. One can compute an importance weight that corresponds to sampling a point on the extended space $(x_1,x_2,...,x_K)$ with target distribution $p(x_1,x_2,...,x_K)$ whose marginal distribution $p(x_1)$ equals the target distribution. The proposal distribution is that which results from the sampling procedure described above. The resulting importance weight is an unbiased estimator for $Z_K/Z_1$, and several runs are averaged together to reduce the variance of the estimate. However, often one is interested in an estimate of $\log Z_K$. The resulting plug-in estimator $\widehat{\log Z_K}=\log(\hat{Z}_K)$ will have a downward bias due to Jensen's inequality. 


If one can obtain samples from the target distribution, the annealing schedule can be run in reverse, starting with a sample from the target distribution, running down the $\beta$ ladder. This approach is called Reverse Annealed Importance Sampling (RAISE)~\cite{raise}. The resulting importance weight is an unbiased estimator for $Z_1/Z_K$. From Jensen's inequality again, the resulting plug-in estimator for $\log Z_K$ will have an upward bias. Thus, by running AIS and RAISE together, one can bound the partition function to an interval. However, since AIS and RAISE are extensions of importance sampling, there must be a large amount of overlap between intermediate distributions for the proposal distribution to sample all regions of high probability in the target distribution. As shown in~\cite{grosse2013annealing}, this is reflected by the bias of the $\log(Z_K/Z_1)$ estimate from AIS
\begin{align}
\mathbb{E}[\widehat{\log(Z_K/Z_1)}]&=\sum_{k=1}^{K-1} \mathbb{E}_{p_{k+1}}\left[\log\left(\frac{f_{k+1}(x)}{f_k(x)}\right)\right]\\
&=\log (Z_K/Z_1)-\sum_{k-1}^{K-1}D_{KL}(p_k||p_{k+1})
\end{align}
This can be troublesome, as if one were to run AIS/RAISE at a given temperature ladder, but found that the gap between estimates was closing too slowly (indicating too few temperatures), the entire procedure would have to be redone with a finer temperature ladder. (It may be the case that one could average the two estimates together to decrease the variance of the final estimate, but non-asymptotically, it is not clear when this would become advantageous.) An advantage of RTS over AIS/RAISE is that a significant overlap of temperatures is not crucial; only enough overlap to permit good mixing is necessary in RTS. Thus, to obtain more accurate estimates with RTS, one needs only to continue collecting samples.
